Efficient Learning in Polyhedral Games via Best Response Oracles

We study online learning and equilibrium computation in games with polyhedral decision sets, a property shared by both normal-form games and extensive-form games (EFGs), when the learning agent is restricted to using a best-response oracle. We show how to achieve constant regret in zero-sum games and $O(T^{1/4})$ regret in general-sum games while using only $O(\log t)$ best-response queries at a given iteration $t$, thus improving over the best prior result, which required $O(T)$ queries per iteration. Moreover, our framework yields the first last-iterate convergence guarantees for self-play with best-response oracles in zero-sum games. This convergence occurs at a linear rate, though with a condition-number dependence. We go on to show a $O(1/\sqrt{T})$ best-iterate convergence rate without such a dependence. Our results build on linear-rate convergence results for variants of the Frank-Wolfe (FW) algorithm for strongly convex and smooth minimization problems over polyhedral domains. These FW results depend on a condition number of the polytope, known as facial distance. In order to enable application to settings such as EFGs, we show two broad new results: 1) the facial distance for polytopes in standard form is at least $\gamma/\sqrt{k}$ where $\gamma$ is the minimum value of a nonzero coordinate of a vertex of the polytope and $k\leq n$ is the number of tight inequality constraints in the optimal face, and 2) the facial distance for polytopes of the form $\mathbf{A}\boldsymbol{x}=\boldsymbol{b},\mathbf{C}\boldsymbol{x}\leq\boldsymbol{d}, \boldsymbol{x}\geq \mathbf{0}$ where $\boldsymbol{x}\in\mathbb{R}^n$, $\mathbf{C}\geq\boldsymbol{0}$ is a nonzero integral matrix, and $\boldsymbol{d}\geq \boldsymbol{0}$, is at least $1/(\|\mathbf{C}\|_\infty\sqrt{n})$. This yields the first such results for several problems such as sequence-form polytopes, flow polytopes, and matching polytopes.

==> algomacros.tex <==
\makeatletter

\patchcmd\algocf@Vline{\vrule}{\vrule \kern-0.4pt}{}{}
\patchcmd\algocf@Vsline{\vrule}{\vrule \kern-0.4pt}{}{}

\apptocmd{\@algocf@start}{\addtolength{\hsize}{1.4em}}{}{}

\let\cref@old@stepcounter\stepcounter
\def\stepcounter#1{%
    \cref@old@stepcounter{#1}%
    \cref@constructprefix{#1}{\cref@result}%
    \@ifundefined{cref@#1@alias}%
    {\def\@tempa{#1}}%
    {\def\@tempa{\csname cref@#1@alias\endcsname}}%
    \protected@edef\cref@currentlabel{%
        [\@tempa][\arabic{#1}][\cref@result]%
        \csname p@#1\endcsname\csname the#1\endcsname}}

\newcounter{algocolumn@line}
\NewDocumentEnvironment {algomulticol} {O{htp!}} {%
    \begin{figure}[#1]%
        \refstepcounter{algocf}%
        \renewcommand\caption[1]{%
            \setlength{\algocf@ruledwidth}{\linewidth}%
            \@algocf@pre@ruled%
            \global\sbox\algocf@capbox{\hskip\AlCapHSkip%
                \setlength{\algocf@lcaptionbox}{\hsize}\addtolength{\algocf@lcaptionbox}{-\AlCapHSkip}%
                \parbox[t]{\algocf@lcaptionbox}{\algocf@captiontext{\fnum@algocf}{##1}}
            }%
            \box\algocf@capbox\kern\interspacetitleruled\hrule%
            width\algocf@ruledwidth height\algotitleheightrule depth0pt\kern\interspacealgoruled%
        }%
        \setcounter{algocolumn@line}{0}
        }{%
        \@algocf@post@ruled%
    \end{figure}%
}

\NewDocumentEnvironment {algocolumn} {O{1}m+b} {%
    \scalebox{#1}{%
        \raisebox{6mm}{%
            \begin{minipage}[t]{#2}%
                \RestyleAlgo{plain}%
                \begin{algorithm}[H]%
                    \setcounter{AlgoLine}{\value{algocolumn@line}}%
                    #3%
                \end{algorithm}%
            \end{minipage}%
        }%
    }%
}{%
    \setcounter{algocolumn@line}{\value{AlgoLine}}%
}

\makeatother

\SetInd{0.3em}{0.6em}
\NewDocumentCommand \SmallIndentation {} {\SetInd{0.25em}{0.75em}}

\setlength{\interspacetitleruled}{3pt}
\newskip\algoinsideskipamount \algoinsideskipamount=2pt plus 0pt minus 0pt
\def\algoinsideskip{\vspace\algoinsideskipamount}
\SetAlgoInsideSkip{algoinsideskip}
\SetAlCapHSkip{1mm}
\setlength{\algomargin}{5mm}

\newcommand{\fnm}[1]{\textsc{#1}}
\newcommand{\kwsty}{\normalfont\bfseries}
\newcommand{\kw}[1]{{\kwsty{}#1}}
\SetAlCapSty{kwsty}
\SetKwSty{kwsty}
\SetFuncSty{fnm}
\SetArgSty{upshape}
\SetFuncArgSty{upshape}
\SetKwComment{Hline}{}{\vspace{-3mm}\textcolor{gray}{\hrule}\vspace{1mm}}
\definecolor{darkgrey}{gray}{0.3}
\definecolor{commentcolor}{gray}{0.5}
\SetKwComment{Comment}{\color{commentcolor}[$\triangleright$\ }{}
\SetCommentSty{}
\SetNlSty{}{\color{black!50}}{}

\SetKwProg{XFn}{function}{}{}
\SetKwProg{XSubr}{subroutine}{}{}
\newcommand{\Fn}[1]{\XFn{\normalfont\fnm{#1}}}
\newcommand{\Subr}[1]{\XSubr{\normalfont\fnm{#1}}}
\SetKwFor{ForEach}{for~each}{do}{end}
\crefalias{AlgoLine}{line}%

\makeatletter
\newcommand{\removelatexerror}{\let\@latex@error\@gobble}
\makeatother
